On the tau invariants in instanton and monopole Floer theories

We unify two existing approaches to the tau invariants in instanton and monopole Floer theories, by identifying $\tau_{\mathrm{G}}$, defined by the second author via the minus flavors $\underline{\operatorname{KHI}}^-$ and $\underline{\operatorname{KHM}}^-$ of the knot homologies, with $\tau_{\mathrm{G}}^{\sharp}$, defined by Baldwin and Sivek via cobordism maps of the $3$-manifold homologies induced by knot surgeries. We exhibit several consequences, including a relationship with Heegaard Floer theory, and use our result to compute $\underline{\operatorname{KHI}}^-$ and $\underline{\operatorname{KHM}}^-$ for twist knots.

==> macros.tex <==
\pdfminorversion=7 % This is to stop the warning about pdfversion 1.7

\pdfsuppresswarningpagegroup=1

\makeatletter
\g@addto@macro\@floatboxreset\centering
\makeatother

\def\mathcenter#1{%
  \vcenter{\hbox{$#1$}}%
}

\allowdisplaybreaks[4]

\addto\extrasamerican{%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \def\subsubsectionautorefname{Section}%
}

\let\fullref\autoref

\newtheorem{theorem}{Theorem}[section]
\newtheorem{maintheorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{maincorollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]

\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{question}{Question}[section]

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem*{convention}{Convention}
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

\makeatletter
\let\c@maintheorem=\c@theorem
\let\c@corollary=\c@theorem
\let\c@maincorollary=\c@theorem
\let\c@proposition=\c@theorem
\let\c@lemma=\c@theorem
\let\c@conjecture=\c@theorem
\let\c@question=\c@theorem
\let\c@remark=\c@theorem
\let\c@example=\c@theorem
\let\c@definition=\c@theorem
\let\c@equation\c@theorem
\makeatother
%
\def\makeautorefname#1#2{\expandafter\def\csname#1autorefname\endcsname{#2}}
\makeautorefname{maintheorem}{Theorem}%
\makeautorefname{maincorollary}{Corollary}%
\makeautorefname{theorem}{Theorem}%
\makeautorefname{corollary}{Corollary}%
\makeautorefname{proposition}{Proposition}%
\makeautorefname{lemma}{Lemma}%
\makeautorefname{conjecture}{Conjecture}%
\makeautorefname{question}{Question}%
\makeautorefname{example}{Example}%
\makeautorefname{remark}{Remark}%
\makeautorefname{definition}{Definition}%

% When referring to equations, print, e.g., Equation (4.8)
% Works by editing the parentheses out of the macro \tagform in amsmath
% and then putting parentheses around \theequation
\numberwithin{equation}{section}
\let\origtheequation\theequation
\makeatletter
\def\tagform@#1{\maketag@@@{\ignorespaces#1\unskip\@@italiccorr}}
\makeatother
\renewcommand{\theequation}{(\origtheequation)}

% Compute adjustments for captionsetup, which are necessary when using pinlabel
\newcommand*{\Alphabet}{ABCDEFGHIJKLMNOPQRSTUVWXYZ1234567890}
\newcommand*{\alphabet}{abcdefghijklmnopqrstuvwxyz1234567890}
\newlength\Lcaph
\newlength\Ldesc
\newlength\Lactualfontsize
\settoheight{\Lcaph}{\Large \Alphabet}
\settodepth{\Ldesc}{\Large \Alphabet \alphabet}
\setlength{\Lactualfontsize}{\dimexpr\Lcaph+\Ldesc\relax}
\newlength\scaph
\newlength\sdesc
\newlength\sactualfontsize
\settoheight{\scaph}{\small \Alphabet}
\settodepth{\sdesc}{\small \Alphabet \alphabet}
\setlength{\sactualfontsize}{\dimexpr\scaph+\sdesc\relax}
\newlength\scrcaph
\newlength\scrdesc
\newlength\scractualfontsize
\settoheight{\scrcaph}{\small \Alphabet}
\settodepth{\scrdesc}{\small \Alphabet \alphabet}
\setlength{\scractualfontsize}{\dimexpr\scrcaph+\scrdesc\relax}


